Oralytics Reinforcement Learning Algorithm

Dental disease is still one of the most common chronic diseases in the United States. While dental disease is preventable through healthy oral self-care behaviors (OSCB), this basic behavior is not consistently practiced. We have developed Oralytics, an online, reinforcement learning (RL) algorithm that optimizes the delivery of personalized intervention prompts to improve OSCB. In this paper, we offer a full overview of algorithm design decisions made using prior data, domain expertise, and experiments in a simulation test bed. The finalized RL algorithm was deployed in the Oralytics clinical trial, conducted from fall 2023 to summer 2024.

==> 00_basics/basics.tex <==
%\alt{Hello Susan, I wrote the two paragraphs you suggested. 1) general intro of main study from viewpoint of RL algorithm and 2) define RL terminology.}
% \sam{We need to start off with a general  intro to Oralytics main study from the viewpoint of RL micro-randomization.  This section should include  duration of main study, decision points in main study, proximal outcome ( definition of quality brushing), definition of when the participant starts the study,  tell reader that participant's are called "participants" in this document.  Define $N$ (sample size for main study).  remind reader that participants will be incrementally recruited at approximately 5 people per two weeks.}
This section documents the development of the reinforcement learning (RL) algorithm for the main study of Oralytics. Reinforcement learning (RL) \cite{sutton2018reinforcement} is an area of machine learning where algorithms learn to select a sequence of decisions in an environment in order to maximize an outcome. In Oralytics, the RL algorithm optimizes the delivery of engagement prompts to participants to maximize their oral self-care behaviors (OSCB) or brushing quality (Section~\ref{brush_quality_def}). We use $N$ to denote the number of participants participating in the main study (sample size). For the main study, the RL algorithm will make decisions for around $N = 70$ participants, where each participant is in the main study for 70 days. The RL algorithm makes decisions everyday at decision points. For Oralytics, the decision points are right before the participant's morning and evening preferred brushing windows (Section~\ref{proximal_outcome_window}). In order to learn which decisions maximizes OSCB for a participant, the RL algorithm updates with participant incoming participant data at update times. For Oralytics, the update times are every Sunday at 4:04 AM PST (Section~\ref{update_cadence}). Participants enter the study incrementally at an expected rate of 5 participants per 2 weeks (See Section~\ref{onboarding_proc} for exact details on the definition of a participant entering the RL part of the study).

% \sam{replace "patient" by "participant" throughout!}

% \sam{in this section define RL terminology: actions (whether to send an intervention prompt), state and reward.  Define feature. define reward function.  Define pure exploration (aka--using prior distribution to sample actions.}
% \sam{define the term, "action" by "binary decision concerning whether to deliver an intervention prompt". Do above in intro.... }
\subsection{Formulating the RL Problem}
To formulate the RL problem, we first define a state, action, and reward. For each of the components, we use subscript $i$ to denote the participant and subscript $t$ to denote the decision point. The state $S_{i, t}$ for participant $i$ at decision point $t$ describes the current context of the participant. We define algorithm state features as relevant features used by the algorithm that provide a summary of state $S_{i, t}$. For example, state features could be weather, location, or amount of dosage in the past week. See Section~\ref{state_features} for the state features for Oralytics. The action $A_{i, t}$ is the decision made by the algorithm for participant $i$ at decision point $t$, based on its policy. A policy is a function that takes in input state $S_{i, t}$ and outputs action $A_{i, t}$. For Oralytics, the action is a binary decision of whether to deliver an engagement prompt ($A_{i, t}=1$) or not ($A_{i, t}=0$) and the policy first calculates the randomization probability $\pi_{i, t}$ of selecting $A_{i, t}=1$ and then uses $\pi_{i, t}$ to sample $A_{i, t}$ from a Bernoulli distribution. That is, $A_{i, t}$ is micro-randomized at time $t$ with randomization probability  $\pi_{i, t}$. For Oralytics, the policy initially undergoes a warm-start period (Section~\ref{onboarding_proc}) where $\pi_{i, t}$ is calculated using the prior distribution (Section~\ref{fitting_prior}). The reward $R_{i, t}$ is a function of the proximal outcome,  designed to  reward the algorithm for selecting good actions for participants.
%The goal of the algorithm is to maximize the total rewards collected for each patient over the entire trial $R = \sum_{t = 1}^T \sum_{i = 1}^N R_{i, t}$.
In Oralytics, the reward is a function of OSCB (proximal health outcome concerning brushing quality) and a proxy for participant burden (cost of current treatment on effectiveness of future treatment) \cite{trella2023reward}. See Section~\ref{reward_def} for more details on the reward designed for Oralytics.

We now describe how the RL algorithm makes decisions and learns throughout the study. The Oralytics algorithm is an \textit{online} RL algorithm which learns and updates throughout the study as new participant data accumulates. 
%This is opposed to the \textit{offline} or batch setting where the algorithm learns before the study starts on previous batch data and is fixed for the entire study. 
An online RL algorithm can be decomposed into two main parts: 1) a  statistical model of the participant (also called  the environment) and 2) a policy (defined above) informed by the participant  model. At decision point $t$, the algorithm observes participant $i$'s observed state $S_{i, t}$ and randomizes action $A_{i, t}$ with randomization probability $\pi_{i, t}$. After the RL algorithm selects $A_{i, t}$, the algorithm then observes the proximal outcome of OSCB $Q_{i, t}$ from the participant. At update times, the RL algorithm updates the model of the participant environment using a history of states, actions, and rewards up to the most recent decision point. 

==> 00_basics/data_and_code.tex <==
\subsection{Available Data}
To inform our design decisions, we use data from ROBAS 2 \cite{info:doi/10.2196/17347} and ROBAS 3, previous dental health studies, and data from the pilot phase of the Oralytics study. All data we use is publicly available:
\begin{itemize}
    \item ROBAS 2: \href{https://github.com/ROBAS-UCLA/ROBAS.2/blob/master/inst/extdata/robas_2_data.csv}{here}
    \item ROBAS 3: \href{https://github.com/ROBAS-UCLA/ROBAS.3/blob/main/data/robas_3_data_complete.csv}{here}
    \item Oralytics Pilot: \href{https://github.com/StatisticalReinforcementLearningLab/oralytics_pilot_data}{here}
\end{itemize}

ROBAS 2 ran with 32 participants where each participant was in the study for 30 days. ROBAS 3 included 31 participants where each participant was in the study for 90 days. The pilot study included 9 participants and the study duration was 35 days. ROBAS 3 and the pilot study used the same sensory suite (i.e., bluetooth toothbrush and sensory-collecting software). This suite is more sophisticated and was able to record brushing pressure to inform OSCB (measure of brushing quality), while the suite for ROBAS 2 could only record brushing duration. A key distinction is that ROBAS 2 and ROBAS 3 had no interventions and the pilot study had interventions selected by a beta version of the RL algorithm. See Table~\ref{robas_3_stats} for additional statistics on the ROBAS 3 data set.

We use the ROBAS 2 data to inform certain design decisions (e.g., cost term parameters-- $b, a_1, a_2$, see Section~\ref{sec:cost_term}-- in reward definition) %\sam{I thought this was only for RL alg in pilot}. \alt{Hello Susan, recall the reward definition Section~\ref{reward_def} was informed using ROBAS 2 data and domain experts (i.e., you). Namely, choosing $b, a_1, a_2$ (on page 19).} 
We use the ROBAS 3 data to design the simulation environment (i.e., fit participant environment models) (Section~\ref{app:sim_env}) and to inform additional design decisions (e.g., slope value of smoothing allocation function). Finally, we use the pilot study to develop the  prior distribution (Section~\ref{fitting_prior}) used by all algorithm candidates (all algorithms are Bayesian and thus require a prior distribution) and to set the participant app opening probability for the simulation environment (Section~\ref{sim_env_variants_open_app}).

One natural approach is to use pilot study data to create another simulation environment. However, the pilot study data is not suitable for creating a separate simulation environment because:

\begin{enumerate}
    \item \textbf{Insufficient Sample Size:} For the pilot study, we only have data on 9 participants.
    \item \textbf{Insufficient Duration of Pilot Study:} Each participant was in the pilot study for 35 days. In contrast, participants will be in the main study for 70 days. When running simulations, we evaluate our RL algorithm in a 70-day study. However, because we only have pilot participant data for 35 days,  the simulation environment built off of pilot data must extrapolate to the final 35 days (i.e., predict OSCB with day in study that was not in the training set).
\end{enumerate}

Both the sample size and duration of the pilot study (35 days)
means that we have data on only 70 decision
points for each of the 9 participants in the pilot study. The small amount of data  per participant  implies that the estimated  parameters in the models are very noisy. 
% Text is too much too early:::  For example, we fit a separate linear model for each of the 9 participants in the pilot study. Notice that in Figure~\ref{fig:ac_model_standard_eff} (5th column, 3rd row) the standardized effect for main treatment effect (effect of sending an intervention prompt) is negative for most participants. We believe this is likely due to noise as  we  expect a nonnegative  average treatment effect for sending an intervention (i.e., participants are unlikely to brush their teeth worse because they received an intervention). 
Therefore, we only use the pilot data to inform: 1) simulated app opening probability (Section~\ref{sim_env_variants_open_app})
and 2) the prior used by algorithm candidates that run in the simulation environment (Section~\ref{fitting_prior}). We continue to use the simulation environment built off ROBAS
3 data to inform design decisions and evaluate the final algorithm going into the Oralytics main study. 

Notice that although we do not have enough data to construct a new simulation
environment, we still use pilot
data to inform the design of the prior distribution for the algorithm. This is because we constructed the prior in collaboration with domain scientists (see Section~\ref{fitting_prior} for more information on constructing the prior). %We first calculated the standard effects across features using the pilot data. For most of the features, the effect size coincided reasonably with domain expertise, and we set prior values with a pre-specified procedure. For features that do not coincide reasonably with domain expertise, the value was overridden and specifically chosen by domain experts.

\begin{table}[H]
\centering
\begin{tabular}{p{0.50\linewidth}p{0.175\linewidth}}
\toprule
Property & ROBAS 3 \\ 
\midrule
Num. Users & 31 \\
\% Sessions with No Brushing  & 53\% \\
Min. OSCB & 0 \\
Max. OSCB & 473 \\
SD. of OSCB & 74.908 \\
Mean of OSCB & 62.750 \\
Median of OSCB & 0.0 \\
\bottomrule
\end{tabular}
\caption{Descriptive statistics for OSCB in the ROBAS 3 data set}
\label{robas_3_stats}
\end{table}

\subsection{Code}
Code for running experiments to finalize design decisions for the RL algorithm can be found in a github repository  \href{https://github.com/StatisticalReinforcementLearningLab/oralytics_algorithm_design}{here}.
% \sam{ask Zara if the consent forms allow this, then if consent forms allow this then ask Billie/Vivek.} \alt{Anna sent email to Zara on 7/11. Waiting on response.} 



==> 00_basics/definitions.tex <==
\subsection{Definitions}
\alt{ANY OTHER HELPFUL DEFINITIONS TO ADD? INSERT ALL NEEDED DEFINITIONS HERE}
\begin{itemize}
\item \label{reg_user_def} \textbf{Definition of Registered User:} A user is registered if the user has completed the on-boarding process with staff (i.e., received a unique study id, downloaded the Oralytics app, and has a first successfully registered brushing session on the cloud platform). Registered users will be added to the RL service database and the RL service will form an initial schedule of actions (70 days) for that user. Notice that a registered user does not mean that the user is currently in the study (please see the below definition for user start day). The RL algorithm \textit{does not update} using registered user's data.
\item \textbf{User Start Date:} We define the user start date as the first day the user \textit{obtains the first schedule of actions}. This happens when 1) the user has successfully registered brushing sessions to the cloud, 2) a schedule has been formed for the user, and 3) they have opened their app and the app has received the schedule. Once these conditions are met, we consider the user as \textit{currently in the study} and the RL service will continue forming schedules of actions and will update the RL algorithm with data tuples from that user.
\item \textbf{User Environment Model:} A user's outcome generating process for simulation environments. For the simulation environment, we simulate a cohort of users (fit on real data) and each user represents a brushing quality generating process.
\end{itemize}

==> 00_basics/main.tex <==
\section{Introduction}

\input{00_basics/basics}
\input{00_basics/data_and_code}

==> 01_alg_stats.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Algorithm Statistics}
\label{alg_stats}

\kwz{I'm thinking to work on getting these statistics for the (1) no incremental recruitment, (2) no action centering setting using pytorch autograd, just to ensure things are working properly. Anna, feel free to ask me any questions you have. Here is code for how I computed gradients for a simpler algorithm: \url{https://github.com/kellywzhang/inference_after_pooling} }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Posterior Sampling}

\noindent \kwz{Let us not do incremental recruitment for now.}

\noindent \kwz{Let's not do action centering for now:}
\begin{equation}
    R_{i, t} = m(S_{i, t})^T \alpha_0 + A_{i, t} f(S_{i, t})^T \beta + \epsilon_{i,t}
\end{equation}
where $\pi_{i,t}$ is the probability that the RL algorithm selects action $A_{i,t} = 1$ in state $S_{i,t}$ for participant $i$ at decision time $t$. $\epsilon_{i,t} \sim \mathcal{N}(0, \sigma_\epsilon^2)$ and there are priors on $\alpha_{0} \sim \mathcal{N}(\mu_{\alpha_0}, \Sigma_{\alpha_0})$, $\beta \sim \mathcal{N}(\mu_{\beta}, \Sigma_{\beta})$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Posterior Distributions}
We let $\theta = [\alpha_0, \beta]$, $\mu_0 = [\mu_{\alpha_0}, \mu_\beta]$, and $\Sigma_0 = \mathrm{Diag}(\Sigma_{\alpha_0}, \Sigma_\beta)$.

\begin{equation*}
    \theta | \history{t}{1:n} \sim \N( \mu_t, \Sigma_t )
\end{equation*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Policy Parameter Estimating Equations}

\begin{equation*}
    \mu_t
    = \hat{V}_{t}^{-1} \frac{1}{n} \left(  \frac{1}{\sigma_\epsilon^2} \sum_{t'=1}^t \sum_{i=1}^n \reward{i}{t'} g(\action{i}{t'}, \state{i}{t'}) +  \Sigma_0^{-1} \mu_0 \right)
\end{equation*}
\begin{equation*}
    V_t = \frac{1}{n} \left( \frac{1}{\sigma_\epsilon^2} \sum_{t'=1}^t
    \sum_{i=1}^n g\big( \action{i}{t'}, \state{i}{t'} \big)^{\otimes 2}
    + \Sigma_0^{-1} \right)
\end{equation*}
where $\Sigma_t = \frac{1}{n} V_t^{-1}$
for $g(\action{i}{t'}, \state{i}{t'}) = \begin{bmatrix} m(\state{i}{t'}) \\ \action{i}{t'} f(\state{i}{t'}) \end{bmatrix}$. We use the notation $x^{\otimes 2} = x x^\top$ for $x \in \real^d$. \\

\noindent Note that
\begin{equation*}
    \mu_t = \argmax_{w} \left\{ - \frac{1}{2 \sigma_\epsilon^2} \frac{1}{n} \sum_{t'=1}^t \sum_{i=1}^n \left( \reward{i}{t} - g(\action{i}{t'}, \state{i}{t'})^\top w \right)^2 - \frac{1}{2} \left( w - \mu_0 \right)^\top \Sigma_0^{-1} \left( w - \mu_0 \right)  \right\}
\end{equation*}
\begin{equation*}
    V_t = \argmax_{V} \left\{ - \frac{1}{2 \sigma_\epsilon^2} \frac{1}{n} \left\| \sum_{i=1}^n \sum_{t'=1}^t g\big( \action{i}{t'}, \state{i}{t'} \big)^{\otimes 2}
	+ \Sigma_0^{-1} - V \right\|_2^2 \right\}
\end{equation*}

\paragraph{Estimating Equation}

For each update time (not each decision time) we need:
\begin{equation*}
	\phi_t \left( \HH_{1:t}^{(i)}; ~ \mu, V \right) 
	= \begin{cases} 
		\frac{1}{\sigma_\epsilon^2} \sum_{t'=1}^t \left( \reward{i}{t'} - g\big( \action{i}{t'}, \state{i}{t'} \big)^\top \mu \right) 
		g\big( \action{i}{t'}, \state{i}{t'} \big)
		- \frac{1}{n} \Sigma_0^{-1} (\mu-\mu_0) \\
		\frac{1}{\sigma_\epsilon^2} \sum_{t'=1}^t g\big( \action{i}{t'}, \state{i}{t'} \big)^{\otimes 2}
		+ \frac{1}{n} \Sigma_0^{-1} - V
    \end{cases}
\end{equation*}

In vector form this is:
\begin{equation*}
	\phi_t \left( \HH_{1:t}^{(i)}; ~ \mu, V \right) 
	= \begin{cases} 
		\frac{1}{\sigma_\epsilon^2} G^T(R - G\mu)
		- \frac{1}{n} \Sigma_0^{-1} (\mu-\mu_0) & \in \mathbb{R}^D \\
		\frac{1}{\sigma_\epsilon^2} G^T G
		+ \frac{1}{n} \Sigma_0^{-1} - V & \in \mathbb{R}^{D x D}
    \end{cases}
\end{equation*}

where $G \in \mathbb{R}^{t x D}$ is a matrix of stacked $g\big( \action{i}{t'}, \state{i}{t'} \big)$'s and $R \in \mathbb{R}^t$ is a vector of stacked $R_{i, t'}$'s.

\begin{itemize}
    \item Every update step, get a $\phi_t\left( \HH_{1:t}^{(i)}; ~ \mu_t, V_t \right)$ for every participant.
    \item $\mu_t, V_t$ solve
    \begin{equation*}
        0 = \frac{1}{n} \sum_{i=1}^n \phi_t \left( \HH_{1:t}^{(i)}; ~ \mu, V \right) 
    \end{equation*}
\end{itemize}

\noindent \kwz{Need $\phi_t \left( \HH_{1:t}^{(i)}; ~ \mu_t, V_t \right)$ for each update step $j$ and $i \in [1 \colon n]$.}
\alt{$\mu_t, \Sigma_t$ are estimators of the mean and variance of the posterior. $\phi_t \left( \HH_{1:t}^{(i)}; ~ \mu_t, V_t \right)$ will give us the mean and variance of the estimators (estimators of posterior mean and posterior variance).}


\paragraph{Derivative of Estimating Equation}
\begin{equation*}
	\dot{\phi}_t \left( \HH_{1:t}^{(i)}; ~ \mu, V \right) 
	= \begin{cases} 
		- \frac{1}{\sigma_\epsilon^2} \sum_{t'=1}^t g\big( \action{i}{t'}, \state{i}{t'} \big)^{\otimes 2}
		- \frac{1}{n} \Sigma_0^{-1} \\
		-I
    \end{cases}
\end{equation*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Policy Derivative Terms}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Action Selection}
\begin{equation*}
    \pi_{t+1} \big( \action{i}{t} = 1, \state{i}{t} = s ; \mu_t, V_t \big) 
\end{equation*}
\begin{equation*}
    =\E_{\theta = [\alpha_0, \beta] \sim \N \left( \mu_t, V_t^{-1} \right) } \left[ \rho( s^\top \beta ) \big| \state{i}{t}=s, \mu_t, V_t \right]
\end{equation*}
\begin{equation}
    \label{eqn:piStandardNormal}
    =\E_{Z \sim \N \left( 0, I \right) } \left[ \rho\left( s^\top \left\{ V_{t, (\beta,\beta)}^{-1/2} Z + \mu_{t, \beta} \right\} \right) \bigg| \state{i}{t}=s, \mu_t, V_t \right]
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Policy Derivative Statistics}

\kwz{Need the statistics for each $i \in [1 \colon n]$ and each $t \in [1 \colon T-1]$:
\begin{equation*}
    \fracpartial{}{\mu} \pi_{t+1} \left( \action{i}{t}, \state{i}{t}; \mu, V \right) \bigg|_{\mu = \mu_t, V = V_t } \in \real^{d}
\end{equation*}
\begin{equation*}
    \fracpartial{}{ V } \pi_{t+1} \left( \action{i}{t}, \state{i}{t}; \mu, V \right) \bigg|_{\mu = \mu_t, V = V_t } \in \real^{d \by d}
\end{equation*}

NEED TO DISCUSS WEIGHTING THESE TERMS and summing}
\alt{We need derivative values for each decision time $t$ and each participant $i$. Each decision time will give you $N$ of $\fracpartial{}{\mu} \pi_{t+1}, \fracpartial{}{ V } \pi_{t+1}$.}

\alt{Sanity check: there's a bunch of 0s for the mu and the V corresponding to $a_0$ because we're not using it.}

\begin{itemize}
	\item Using display \eqref{eqn:piStandardNormal}, the derivative $\fracpartial{}{\mu } \pi_t \big( \action{i}{t} = 1, \state{i}{t} = s ; \mu, V \big) \in \real^{d}$ is
	\begin{multline*}
		\fracpartial{}{ \mu } \pi_t \big( 1, s ; \mu, V  \big) \\
		= \begin{cases}
		    0 & \mathrm{for~first~dim}(\alpha_0)\mathrm{~dimensions} \\
			\E_{Z \sim \N( 0, I) } \left[ \dot{\rho} \left( s^\top \left\{ V_{(\beta,\beta)}^{-1/2} Z + \mu_{\beta} \right\} \right) s
			\bigg| \state{i}{t} = s, \mu, V \right] & \mathrm{for~last~dim}(\beta)\mathrm{~dimensions}
		\end{cases}
	\end{multline*}
	\item The derivative $\fracpartial{}{V} \pi_t \big( \action{i}{t} = 1, \state{i}{t} = s ; \mu, V \big)$ is a scalar.
	\begin{multline*}
		\fracpartial{}{ V } \pi_t \left( \action{i}{t} = 1, \state{i}{t} = s ; \mu, V \right) \\
		= \begin{cases}
		    0 & \mathrm{for~dim~} V_{(\alpha,\alpha)}, V_{(\alpha,\beta)}, V_{(\beta,\alpha)} \\
		    \E_{Z \sim \N( 0, I) } \left[ \dot{\rho} \left( s^\top \left\{ V_{(\beta,\beta)}^{-1/2} Z + \mu_{\beta} \right\} \right)
		    Z s^\top \fracpartial{}{V} V^{-1/2}
		    \bigg| \state{i}{t} = s, \mu, V \right] & \mathrm{for~dim~} V_{(\beta,\beta)}
		\end{cases}
	\end{multline*}
	Above I use that $\fracpartial{}{V} s^\top V Z = Z s^\top$ (recall $s, Z$ are vectors); see \href{https://www.math.uwaterloo.ca/~hwolkowi/matrixcookbook.pdf}{matrix cookbook} display (71).
	\kwz{I'm hoping that we can automatically get gradients for $\fracpartial{}{V} V^{-1}$ using pytorch eigendecomposition. Since $V$ is positive definite, we can find orthonormal matrix $Q$ and diagonal matrix $\Lambda$ such that $V = Q \Lambda Q^{-1}$ and $V^{-1/2} = Q \Lambda^{-1/2} Q^{-1}$}
	%Above I use that $\fracpartial{}{V} s^\top V Z = Z s^\top$ (recall $s, Z$ are vectors) and $\fracpartial{}{x} V^{-1} = - V^{-1} \left( \fracpartial{}{x} V \right) V^{-1}$ for a scalar $x$; see \href{https://www.math.uwaterloo.ca/~hwolkowi/matrixcookbook.pdf}{matrix cookbook} displays (71) and (59) respectively.
\end{itemize}

==> 01_sample_size.tex <==
\subsection{Sample Size Calculation}
\label{sample_size_calc}

\alt{KELLY PLEASE DUMP HERE! Could you also specify if this sample size calculation is for the pilot study or for the real study?}

==> 04_total_vars.tex <==
\subsection{Simulation Environment Variants}
\label{all_exp_env_vars}
There are 12 total environment variants. The variant axes are:
\begin{itemize}
    \item \textbf{Environment Feature Space:} We consider two environments, stationary vs. non-stationary (see more information in Section~\ref{baseline_features}).
    \item \textbf{Level of participant Habituation:} We consider three shrinkage factors of $E = \{0, 0.5, 0.8\}$ (see more information in Section~\ref{sim_env_variants_delayed_effs}).
    \item \textbf{Population-Level Effect Sizes:} We consider a reasonable small effect size (shrinkage value $\zeta=\frac{1}{8}$) and a less small effect size (shrinkage value $\zeta=\frac{1}{4}$) (see more information in Section~\ref{treatment_eff_sizes}).
    % \item \textbf{Probability of participants Opening the App:} We consider two schemes for participants opening the app: 1) all participants open the app everyday and 2) participants open the app with probability 0.8 if they receive a message that day and a probability of 0.2 if they do not. (see more information in Section~\ref{sim_env_variants_open_app})
\end{itemize}



==> archive/alg_type_experiments.tex <==
\section{Algorithm Type Experiments}
We evaluate the RL algorithm candidates in each of the environment variants. For our experiments, we simulate four users entering the study every week (incremental recruitment). To simulate a study, we draw $N = 72$ users (approximately the expected sample size for the Oralytics study) with replacement and cluster them by their entry date into the simulated study. The algorithms for each cluster are updated weekly with the first update taking place after one week (at decision time $t=14$ for each cluster).

We use a contextual bandit framework with Thompson sampling, full-pooling,
a Bayesian Linear Regression, $[0.1, 0.9]$ clipping values, and an informative prior fit using ROBAS 2 data. In these experiments, we test an action centering vs. a no action centering reward approximating function and a steep versus a flat slope for the smoothing allocation function.

\begin{table}[H]
%    \centering
\begin{tabular}{lll}
\toprule
    \textbf{STAT\_LOW\_R:} Stationary Base Model, $E=0$  \\
    \midrule
    \textbf{NON\_STAT\_LOW\_R} Non-Stationary Base Model, $E=0$ \\
    \midrule
    \textbf{STAT\_MED\_R:} Stationary Base Model, $E=0.5$ \\
    \midrule
    \textbf{NON\_STAT\_MED\_R} Non-Stationary Base Model, $E=0.5$ \\
    \midrule
    \textbf{STAT\_HIGH\_R} Stationary Base Model $E=0.8$ \\
    \midrule
    \textbf{NON\_STAT\_HIGH\_R} Non-Stationary Base Model, $E=0.8$ \\ 
\bottomrule
\end{tabular}
\caption{{\textbf{Six Environment Variants}}.
We consider two environment base models (stationary and nonstationary) and three shrinkage values $E$ (low $E = 0$, medium $E = 0.5$, and high $E = 0.8$) Shrinkage values shrink the user-specific effect size if a user receives too many messages. Low values of $E$ means that users are more susceptible to habituation than higher values of $E$.}
\label{tab:env_variants}
\end{table}

\begin{table}[H]
%    \centering
\begin{tabular}{lll}
\toprule
    \textbf{AC Flat:} Action-Centering, $B=0.515$ \\
    \midrule
    \textbf{AC Steep:} Action-Centering, $B=5$ \\
    \midrule
    \textbf{No AC Flat} No Action-Centering, $B=0.515$ \\
    \midrule
    \textbf{No AC Steep} No Action-Centering, $B=5$ \\ 
\bottomrule
\end{tabular}
\caption{{\textbf{Four Algorithm Candidates}}.
We consider two types of Bayesian Linear Regression reward approximating functions and two slope values $B$ for the smoothing allocation function for the RL algorithm.}
\label{tab:alg_candidates}
\end{table}

\begin{table}[H]
\begin{tabular}{lllll}
\toprule
\multicolumn{1}{c}{} & \multicolumn{4}{c}{Average Rewards} \\
\toprule
Environments & AC Flat &  AC Steep & No AC Flat & No AC Steep \\
\midrule
STAT\_LOW\_R & \textbf{62.659 (0.457)} & 62.407 (0.449) &  58.800 (0.513) & 58.341 (0.504) \\
STAT\_MED\_R & \textbf{62.880 (0.470)} & 62.506 (0.454) &  59.193 (0.464) & 58.761 (0.456) \\
STAT\_HIGH\_R & \textbf{63.683 (0.471)} & 63.268 (0.471) &  59.628 (0.481) & 59.062 (0.465) \\
NON\_STAT\_LOW\_R & \textbf{60.969 (0.409)} & 60.240 (0.439) &  58.389 (0.461) & 57.753 (0.488) \\
NON\_STAT\_MED\_R & \textbf{61.243 (0.426)} & 60.881 (0.437) &  58.387 (0.455) & 58.316 (0.455) \\
NON\_STAT\_HIGH\_R & \textbf{61.631 (0.435)} & 61.382 (0.436) &  58.704 (0.426) & 57.903 (0.457) \\

\midrule
\multicolumn{1}{c}{} & \multicolumn{4}{c}{25th Percentile Rewards} \\
\midrule
Environments &  AC Flat &  AC Steep & No AC Flat & No AC Steep \\
\midrule
STAT\_LOW\_R & \textbf{24.940 (1.233)} & 23.417 (1.109) &  22.275 (1.120) & 22.243 (1.001) \\
STAT\_MED\_R & \textbf{24.360 (1.177)} & 23.776 (1.150) &  22.336 (1.069) & 22.617 (1.108) \\
STAT\_HIGH\_R & \textbf{25.030 (1.218)} & 24.709 (1.270) &  22.825 (1.129) & 22.906 (1.144) \\
NON\_STAT\_LOW\_R & \textbf{27.059 (0.978)} & 25.737 (1.001) &  25.060 (0.901) & 25.103 (0.956) \\
NON\_STAT\_MED\_R & \textbf{27.098 (0.967)} & 26.269 (1.024) &  25.905 (0.914) & 26.025 (0.936) \\
NON\_STAT\_HIGH\_R & \textbf{26.911 (1.028)} & 26.377 (1.017) &  26.444 (0.918) & 25.105 (0.948) \\
\bottomrule
\end{tabular}
\caption{{Average and 25th Percentile Rewards.}
The naming convention for environment variants and algorithm candidates are found in Table~\ref{tab:env_variants} and Table~\ref{tab:alg_candidates}. The best performing algorithm candidate in each environment variant is bolded.}
\end{table}

\subsection{Takeaways}
\begin{itemize}
    \item Bayesian Linear Regression with action-centering outperfroms Bayesian Linear Regression without action-centering.
    \item Steeper slope $B=0.515$ and flatter slope $B=5$ perform similarly.
\end{itemize}

==> archive/app_opening_issue.tex <==
\newpage
\section{Dealing with App Opening Issue}
\subsection{Issue}
We have a cloud-based system for our RL algorithm that will be run in a clinical trial. The cloud-based system consists of 1) a sensory collecting device (i.e. Bluetooth toothbrush), 2) cloud server (performs inference and training), and 3) device that relays the current action to the user (i.e. mobile phone app). While cloud-based systems offer efficiencies and other advantages, it poses a major issue: \textit{the algorithm can only relay the most recent action when the user opens the app.} (Note: the algorithm will always obtain current state and reward regardless of user opening the app because the sensory collecting device directly communicates with the cloud server.) This is because to protect user security, both iOS and Android put strict limits on background execution, preventing the process from running any code \cite{android:background, apple:background}. Requiring the user to open their app multiple times a day is unrealistic. Therefore, we want to modify the RL algorithm to deal with the case where the user does not open the app.

% In addition, this means that the effectiveness of the RL algorithm is now conflated with the user opening the application.

\section{Approach}
To mitigate this issue, we both modify the RL algorithm and set a staff protocol to encourage users to open the app.

\subsection{Modified RL Algorithm}
Ideally, we want each action selection to be based on the most current data. However, in case the user does not open the app we have the RL algorithm provide a 14-day schedule of actions starting with the current decision time $t$. The RL algorithm will return a matrix in $\mathbb{R}^{14 x 2}$ where each row represents the action selected for the user $i$'s morning and evening decision times for that day. To select actions for day 1, we will use the current state $S_{i, t}, S_{i, t + 1}$ (See Section~\ref{app:rl_alg_features}). For decision times $j = t + 2, t + 3,..., t + 26, t + 27$ we will use a different state space (See Section~\ref{app:modified_rl_features}).

\subsubsection{Feature Space of the RL Algorithm}
\label{app:rl_alg_features}
$S_{i,t} \in \mathbb{R}^d$ represents the $i$th participant's state at decision time $t$, where $d$ is the number of features describing the participant's state.

\begin{enumerate}
    \item Bias / Intercept Term $\in \mathbb{R}$
    \item Time of Day (Morning/Evening) $\in \{0, 1\}$
    % [0, 180]
    \item Exponential Average of Brushing Over Past 7 Days (Normalized) $\in \mathbb{R}$
    \item Exponential Average of Messages Sent Over Past 7 Days $\in [0, 1]$
    \item Prior Day Phone Engagement $\in \{0, 1\}$
    \item Weekend Indicator (Weekday/Weekend) $\in \{0, 1\}$
\end{enumerate}
Features 3 and 4 are $\bar{B} = c_{\gamma}\sum_{j = 1}^{14} \gamma^{j-1} B_{i, t - j}$ and $\bar{A} = c_{\gamma}\sum_{j = 1}^{14} \gamma^{j-1} A_{i, t - j}$.

\subsubsection{Modified Feature Space of the RL Algorithm}
\label{app:modified_rl_features}
Notice the features specified in Section~\ref{app:rl_alg_features} we know definitely except for feature 3. The modified state space is:
\begin{enumerate}
    \item Bias / Intercept Term $\in \mathbb{R}$
    \item Time of Day (Morning/Evening) $\in \{0, 1\}$
    % [0, 180]
    \item Most Recent Exponential Average of Brushing Over Past 7 Days (Normalized) $\in \mathbb{R}$
    \item Indicator of staleness of state (e.g. number of days since user has opened the app)
    \item Exponential Average of Messages Sent Over Past 7 Days $\in [0, 1]$
    \item Prior Day Phone Engagement $\in \{0, 1\}$
    \item Weekend Indicator (Weekday/Weekend) $\in \{0, 1\}$
\end{enumerate}

\subsection{Staff Protocol}
We also employ a protocol to encourage users to open the app:

\begin{enumerate}
    \item The intervention prompts themselves are designed to encourage users to open the app
    \item the staff will send users a text message if they do not open the app for 5 days and a call if they don't open the app 5 days after getting a text message.
    \item there is a 30 day touch point and an exit interview (user is paid for both sessions) where staff can ask the user to open the app
\end{enumerate}

\section{Feedback}
We would like feedback on:
\begin{itemize}
    \item how do we combine the RL algorithm that selects actions for the current day with the RL algorithm that selects actions for the next 13 days? (i.e. the algorithm's state space will zero out certain covariates if it's the most current day)
\end{itemize}

==> archive/notes.tex <==
\section{Notes from Jan 18}
% \includegraphics[scale=0.2]{figures/app_issue.jpeg}

\subsection{App Issue: Need a record of which schedule was executed even if no message was sent}
We need a way to know what action from which schedule was executed, depending on when the user opens the app. At first we thought to just check if the user opened the app at all during the past 24 hours. However, this could be incorrect. For example, if the user opens the app at 4PM, they will get the most recent schedule in time for the evening session but they missed it for the morning session.

Therefore it's not enough to know if the user opened the app in the past 24 hours, but we need to know which actions got scheduled for the user (including actions that don't send a message because we need to match the action selection probability with the action when updating the RL algorithm). 

Hayk currently gives me information about which messages were scheduled and delivered to the user. This is helpful in knowing the schedule for the cases where a message is sent, but I also need to know the schedule id for a brushing session where we don't send a message. 

\bo{If this issue is not resolved, we will not know what action selection probability was used to select actions.} \\

\textbf{Potential Solution: } I have asked Hayk if he could also give me information about which schedule was used even if that action is 0. He has not responded. I am concerned that this fix may not be ready in time for the pilot.

\subsection{RL Algorithm Training Procedure}
\bo{Does below seem reasonable?}
\begin{itemize}
    \item Prior to the $t^{th}$ decision time (assume this is a morning decision time), the algorithm creates a schedule for the next week. Let's call this schedule of actions $A_{i,t}^{(t)}, A_{i,t+1}^{(t)}, \dots, A_{i,t+13}^{(t)}$; there are 14 actions since there are two decision times a day. We include a superscript because this is the schedule of actions formed with the information known up to decision time $t$.
    \begin{itemize}
        \item We now discuss the state that that is used to select these 14 actions. Recall the state features are intercept, time of day, exponential average of previous brushing, exponential average of messages sent over past 7 days
        \item The only state feature that is missing when selecting actions for future days (i.e., decision times $t'$ for $t' > t+1$) is the exponential average of previous brushing. We impute this quantity with the most recently seen exponential average of previous brushing. We call these imputed states $S_{i,t'}^{(t)}$ for $t' > t+1$.
        \item We call the action selection probabilities used to select these actions $\pi_{i,t}^{(t)}, \pi_{i,t+1}^{(t)}, \pi_{i,t+2}^{(t)}, \pi_{i,t+3}^{(t)}, \dots \pi_{i,t+13}^{(t)}$, these uses states $S_{i,t}^{(t)}, S_{i,t+1}^{(t)}, S_{i,t+2}^{(t)}, S_{i,t+3}^{(t)}, \dots, S_{i,t+13}^{(t)}$ to form these probabilities respectively.
    \end{itemize}
    \item Suppose two days pass and the schedule has not been updated, so actions $A_{i,t}^{(t)}, A_{i,t+1}^{(t)}, A_{i,t+2}^{(t)}, A_{i,t+3}^{(t)}$ have been executed;  We need to update the algorithm to form a new schedule in case the user opens the app.
    \begin{itemize}
        \item Recall the Bayesian linear regression model (just copied from earlier in this document):
        \begin{equation}
            R_{i, t} = m(S_{i, t})^T \alpha_0 + \pi_{i,t} f(S_{i, t})^T \alpha_1 + (A_{i, t} - \pi_{i, t}) f(S_{i, t})^T \beta + \epsilon_{i,t}
        \end{equation}
        where $\pi_{i,t}$ is the probability that the RL algorithm selects action $A_{i,t} = 1$ in state $S_{i,t}$ for participant $i$ at decision time $t$. $\epsilon_{i,t} \sim \mathcal{N}(0, \sigma^2)$ and there are priors on $\alpha_{0} \sim \mathcal{N}(\mu_{\alpha_0}, \Sigma_{\alpha_0})$, $\alpha_{1} \sim \mathcal{N}(\mu_{\beta}, \Sigma_{\beta})$, $\beta \sim \mathcal{N}(\mu_{\beta}, \Sigma_{\beta})$.
        %%%%%%%%%%%%
        \item Recall the actions $A_{i,t+2}^{(t)}, A_{i,t+3}^{(t)}$ were selected using imputed states $S_{i,t+2}^{(t)}, S_{i,t+3}^{(t)}$
        \item We are thinking to \textit{not} use the imputed states $S_{i,t+2}^{(t)}, S_{i,t+3}^{(t)}$, but the true states $S_{i,t+2}^{(t+2)}, S_{i,t+3}^{(t+2)}$, which the algorithm will have knowledge of, to update the algorithm.
        %%%%%%%%%%%%
        \item However, for the action centering component of the algorithm, we will use the probabilities that were actually used to select the actions $\pi_{i,t+2}^{(t)}, \pi_{i,t+3}^{(t)}$ (which were formed using imputed states $S_{i,t+2}^{(t)}, S_{i,t+3}^{(t)}$)
        \item \bo{Does this seem reasonable?}   \sam{Yes the learning alg should always use the most accurate states possible!   This should happen even if the action selection strategy is forced to use a stale state.}
    \end{itemize}
\end{itemize}

==> archive/smoothing_function_experiments.tex <==
\subsubsection{Simulations}
We evaluate the RL algorithm candidates in each of the environment variants. For our experiments, we simulate four users entering the study every week (incremental recruitment). To simulate a study, we draw $N = 72$ users (approximately the expected sample size for the Oralytics study) with replacement and cluster them by their entry date into the simulated study. The algorithms for each cluster are updated weekly with the first update taking place after one week (at decision time $t=14$ for each cluster).

We use a contextual bandit framework with Thompson sampling, full-pooling,
a Bayesian Linear Regression with action centering reward approximating function, and an informative prior fit using ROBAS 2 data.

\begin{table}[H]
%    \centering
\begin{tabular}{lll}
\toprule
    \textbf{STAT\_LOW\_R:} Stationary Base Model, $E=0$  \\
    \midrule
    \textbf{NON\_STAT\_LOW\_R} Non-Stationary Base Model, $E=0$ \\
    \midrule
    \textbf{STAT\_MED\_R:} Stationary Base Model, $E=0.5$ \\
    \midrule
    \textbf{NON\_STAT\_MED\_R} Non-Stationary Base Model, $E=0.5$ \\
    \midrule
    \textbf{STAT\_HIGH\_R} Stationary Base Model $E=0.8$ \\
    \midrule
    \textbf{NON\_STAT\_HIGH\_R} Non-Stationary Base Model, $E=0.8$ \\ 
\bottomrule
\end{tabular}
\caption{{\textbf{Six Environment Variants}}.
We consider two environment base models (stationary and nonstationary) and three shrinkage values $E$ (low $E = 0$, medium $E = 0.5$, and high $E = 0.8$) Shrinkage values shrink the user-specific effect size if a user receives too many messages. Low values of $E$ means that users are more susceptible to habituation than higher values of $E$.}
\label{tab:env_variants}
\end{table}

\begin{table}[H]
%    \centering
\begin{tabular}{lll}
\toprule
    \textbf{Wide Steep:} Clipping Values = [0.1, 0.9], $B=0.515$ \\
    \midrule
    \textbf{Wide Flat:} Clipping Values = [0.1, 0.9], $B=0.343$ \\
    \midrule
    \textbf{Narrow Steep} Clipping Values = [0.35, 0.75], $B=0.515$ \\
    \midrule
    \textbf{Narrow Flat}  Clipping Values = [0.35, 0.75], $B=0.343$\\ 
\bottomrule
\end{tabular}
\caption{{\textbf{Four Algorithm Candidates}}.
We consider two types of clipping values $[\pi_{\min}, \pi_{\max}]$ and two slope values $B$ for the smoothing allocation function for the RL algorithm.}
\label{tab:alg_candidates}
\end{table}

\subsubsection{Results}
\begin{table}[H]
\begin{tabular}{lllll}
\toprule
\multicolumn{1}{c}{} & \multicolumn{4}{c}{Average Rewards} \\
\toprule
Environments &  Wide Steep &  Wide Flat & Narrow Steep & Narrow Flat \\
\midrule
STAT\_LOW\_R & 62.457 (0.467) & \textbf{62.704 (0.449)} &  60.897 (0.434) &  60.976 (0.444) \\
STAT\_MED\_R & 63.045 (0.425) & \textbf{63.077 (0.462)} &  61.233 (0.435) &  61.426 (0.441) \\
STAT\_HIGH\_R & 63.214 (0.471) & \textbf{63.328 (0.471)} &  61.595 (0.449) &  61.568 (0.450) \\
NON\_STAT\_LOW\_R & 60.988 (0.409) & \textbf{61.210 (0.422)} &  59.647 (0.405) &  59.617 (0.404) \\
NON\_STAT\_MED\_R & 61.454 (0.439) & \textbf{61.545 (0.409)} &  60.135 (0.409) &  59.889 (0.397) \\
NON\_STAT\_HIGH\_R & 61.586 (0.426) & \textbf{61.933 (0.433)} &  60.113 (0.418) &  60.280 (0.405) \\

\midrule
\multicolumn{1}{c}{} & \multicolumn{4}{c}{25th Percentile Rewards} \\
\midrule
Environments &  Wide Steep &  Wide Flat & Narrow Steep & Narrow Flat \\
\midrule
STAT\_LOW\_R & \textbf{24.228 (1.147)} & 24.020 (1.136) &  23.236 (1.110) &  22.749 (1.030) \\
STAT\_MED\_R & \textbf{24.164 (1.114)} & 23.989 (1.163) &  23.586 (1.119) &  23.816 (1.077) \\
STAT\_HIGH\_R & 24.817 (1.241) & \textbf{25.187 (1.220)} &  24.137 (1.157) &  24.679 (1.191) \\
NON\_STAT\_LOW\_R & 26.121 (0.985) & \textbf{26.985 (0.989)} &  26.979 (0.910) &  26.140 (0.936) \\
NON\_STAT\_MED\_R & 26.976 (1.010) & \textbf{27.384 (0.980)} &  26.460 (0.967) &  26.994 (0.932) \\
NON\_STAT\_HIGH\_R & 26.326 (0.956) & \textbf{27.366 (0.966)} &  26.469 (0.929) &  26.741 (0.954) \\
\bottomrule
\end{tabular}
\caption{{Average and 25th Percentile Rewards.}
The naming convention for environment variants and algorithm candidates are found in Table~\ref{tab:env_variants} and Table~\ref{tab:alg_candidates}. The best performing algorithm candidate in each environment variant is bolded.}
\end{table}

\paragraph{\textbf{Takeaways}}
\begin{itemize}
    \item $[0.1, 0.9]$ Wide clipping values perform better than $[0.35, 0.75]$ narrow clipping values
    \item Steeper slope $B=0.515$ and flatter slope $B=0.343$ perform similarly.
\end{itemize}
